Timely Fusion of Surround Radar/Lidar for Object Detection in Autonomous Driving Systems

Fusing Radar and Lidar sensor data can fully utilize their complementary advantages and provide more accurate reconstruction of the surrounding for autonomous driving systems. Surround Radar/Lidar can provide 360-degree view sampling with the minimal cost, which are promising sensing hardware solutions for autonomous driving systems. However, due to the intrinsic physical constraints, the rotating speed of surround Radar, and thus the frequency to generate Radar data frames, is much lower than surround Lidar. Existing Radar/Lidar fusion methods have to work at the low frequency of surround Radar, which cannot meet the high responsiveness requirement of autonomous driving systems.This paper develops techniques to fuse surround Radar/Lidar with working frequency only limited by the faster surround Lidar instead of the slower surround Radar, based on the state-of-the-art object detection model MVDNet. The basic idea of our approach is simple: we let MVDNet work with temporally unaligned data from Radar/Lidar, so that fusion can take place at any time when a new Lidar data frame arrives, instead of waiting for the slow Radar data frame. However, directly applying MVDNet to temporally unaligned Radar/Lidar data greatly degrades its object detection accuracy. The key information revealed in this paper is that we can achieve high output frequency with little accuracy loss by enhancing the training procedure to explore the temporal redundancy in MVDNet so that it can tolerate the temporal unalignment of input data. We explore several different ways of training enhancement and compare them quantitatively with experiments.

==> backup.tex <==

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{figures/pipeline.pdf}
\caption{Processing Graph of An Autonomous Driving System}
\label{pipeline}
\end{figure}

\begin{itemize}
    \item which node to be time-triggered, which to be event triggered
    
    \item rate tuning by changing the period of time-triggered nodes
\end{itemize}

Requirement
\begin{itemize}
\item The reaction time of the braking must be under certain threshold, which is decided by control module
The minimal reaction time is at least XXX. No buffer overwrite (finish within period?)

\item The sample separation is at most XXX, the age of information is at most XXX. The planning should be done as frequent as possible.

\item Emergency control

\item the control module will compute the reaction time requirement of the next frame, according to the vehicle status, including the speed, the result of the fast object tracking

\item the rate adjuster will compute new period and send it 
to the two perception module
\end{itemize}



Approach:
\begin{itemize}
\item Naturally, we should check whether the worst-case if it is feasible.

\item However, this is not enough, need to consider the mode switch

\begin{itemize}
\item Do we need to design a protocol to control how the sampling separation of 2d perception changes? If not, then we may assume the 


\end{itemize}

\end{itemize}

==> sections/eval.tex <==
\section{Experiments}
\textbf{Dataset preparation.} Following MVDNet\cite{qian2021robust}, we use the Oxford Radar Robotcar\cite{barnes2020oxford} dataset for our experiments. The dataset has 8,862 sample pairs of Lidar and Radar frames, which are split into training and testing tests (7,071 and 1,791 for each respectively) without being overlapped in terms of geography. We prepare the data by using the timestamps of Lidar frames as index and pair it with the latest generated Radar frame. As mentioned in the section \ref{instinsic}, significant scan delay in Radar results in non-synchronization with Lidar and frame-wise misalignment. \textbf{Therefore, there is an $offset$ between our paired Radar/Lidar frames.} In the experiments, we configure the $offset = {\{0, 0.3\Delta t^r, 0.5\Delta t^r, 0.7\Delta t^r\}}$ ($\Delta t^r$ is the latency of a Radar scan). The larger value of \emph{offset}, the longer delay between Radar and Lidar. 

\textbf{Evaluation of proposed fusion method for time asynchronous data.} We prepare the paired Radar and Lidar frames based on our proposed fusion policy and train the MVDNet model on the paired data with different \emph{offset}. Table \ref{AP} shows the detection AP of the various MVDNet models. As expected, for the testing data with offset, MVDNet models trained on paired data with offset consistently outperform the original MVDNet model trained on the time-synchronized data (offset\_0 testing data). The result demonstrates that our proposed fusion method is able to achieve very good vehicle detection accuracy when the paired Radar and Lidar frames are not synchronized in time. In our scenario, the Radar frame is usually behind Lidar frame in time. The result also solves the first issue we mentioned in section \ref{sensorfusion}. \textbf{On the one hand, our fusion method can increase the fusion frequency to Lidar sensor's sampling frequency because it depends on the timestamps of faster Lidar rather than lower Radar. On the other hand, our fusion method can achieve good fusion and detection performance.}



% the skipping some historical frames policy
\textbf{Evaluation of historical frames selection strategies.} As shown in Table \ref{skip}, when setting the \emph{history\_num} = 2, the accuracy of our skipping historical frames strategy is slightly better than that of method using consecutive historical frames. But, the sensor frames in our method can represent more information, which is equal to the setting of \emph{history\_num} = 4. When comparing our skipping history frames strategy (\emph{history\_num} = 2) with original method using 4 consecutive historical frames, the accuracy of our method drops a bit, but is within the acceptable range. After all, our skipping strategy uses almost half as much data to represent the same amount of information, and there is a trade off between \emph{history\_num} and accuracy. The less frames we used, the less latency the model to process it. Therefore, our skipping historical frames selection strategy is demonstrated to be an efficient trade off between the accuracy and runtime.


\begin{table*}[ht]
\centering
\caption{Overall performance of historical frames selection strategy: AP of oriented bounding boxes in bird's eye view.}
\label{skip}
\begin{tabular}{|lc|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Method}} & \begin{tabular}[c]{@{}c@{}}Testing \\ Data\end{tabular} & \multicolumn{3}{c|}{offset\_0.3}                                & \multicolumn{3}{c|}{offset\_0.5}                                & \multicolumn{3}{c|}{offset\_0.7}                                \\ \cline{2-11} 
\multicolumn{1}{|c|}{}                        & IoU                                                     & \multicolumn{1}{c|}{0.5}   & \multicolumn{1}{c|}{0.65}  & 0.8   & \multicolumn{1}{c|}{0.5}   & \multicolumn{1}{c|}{0.65}  & 0.8   & \multicolumn{1}{c|}{0.5}   & \multicolumn{1}{c|}{0.65}  & 0.8   \\ \hline
\multicolumn{2}{|l|}{No skipping, history\_num=4}                                                       & \multicolumn{1}{c|}{0.888} & \multicolumn{1}{c|}{0.860} & 0.707 & \multicolumn{1}{c|}{0.89}  & \multicolumn{1}{c|}{0.863} & 0.684 & \multicolumn{1}{c|}{0.886} & \multicolumn{1}{c|}{0.718} & 0.662 \\ \hline
\multicolumn{2}{|l|}{No shipping, history\_num=2}                                                       & \multicolumn{1}{c|}{0.883} & \multicolumn{1}{c|}{0.863} & 0.72  & \multicolumn{1}{c|}{0.885} & \multicolumn{1}{c|}{0.864} & 0.718 & \multicolumn{1}{c|}{0.869} & \multicolumn{1}{c|}{0.856} & 0.712 \\ \hline
\multicolumn{2}{|l|}{Skipping, history\_num=2}                                                          & \multicolumn{1}{c|}{0.885} & \multicolumn{1}{c|}{0.865} & 0.715 & \multicolumn{1}{c|}{0.887} & \multicolumn{1}{c|}{0.886} & 0.721 & \multicolumn{1}{c|}{0.887} & \multicolumn{1}{c|}{0.867} & 0.71  \\ \hline
\end{tabular}
\end{table*}



% the align_offset_n policy
{\color{red} To be modified here.} \textbf{Evaluation of historical frames matching strategies.} As shown in Table \ref{align}, for each n=\{0,0.3,05,0.7\}, the MVDNet model trained on align\_offset\_n achieves higher accuracy on align\_offset\_n testing data than that the MVDNet model trained on offset\_n training dataset evaluated on offset\_n testing data within various IoUs. The strategy of aligning all historical Radar/Lidar frames to be synchronized achieves average gains of 6.67\%, 1.67\% and 1.93\% with IoU from 0.5 to 0.8, demonstrating that our matching strategy has improved the accuracy.
 








==> sections/unused.tex <==
\label{instinsic}
With the wavelength, the Radar can detect object at long distance and through fog or clouds. Lidar is a compact solution that enables a high level of accuracy for 3D mapping within a short distance.
Because Radar wave has a much longer wavelength and less attenuation than the light waves of Lidar, generally the rotation speed of Radar is slower than Lidar\cite{cen2018precise}. Due to the limitation of Rotation speed, there are fewer Radar sensors that can rotate \ang{360} are used in autonomous vehicle than Lidar, among which the most mainstream surround Radar is  NavTech CTS350-X Radar. NavTech CTS350-X Radar scans the \ang{360} filed of view at a step of \ang{0.9} every 0.25 s. In comparison, the widely used Velodyne HDL-32E Lidar rotates at a step of \ang{0.33} every 0.05s. Our paper aims to solve the limitation of slow rotation speed of surround Radar in multi-sensor fusion.






\subsection{Notations} 
Table \ref{concept} lists some concepts used in this paper. 
Radar samples at frequency $F_r$ Hz and rotates \ang{360} every $1/F_r$ time, generating each R\_raw\_frame with a \ang{360} filed of view. Lidar samples at a faster frequency $F_l$  Hz ($F_l \textgreater F_r$) and rotates \ang{360} every $1/F_l$ time, generating each L\_raw\_frame.  Both Radar and Lidar share the same coordinate origin. Given Radar intensity maps and Lidar point clouds, we aim to detect the vehicle in bird-eye-view (BEV) projection maps.

Specially, we are given $N$ R\_raw\_frames denoted by $X_r = \{x_r^i\}_{i=1}^N$ where the arrival frequency of each raw frame is $F_r$ Hz. $M$ L\_raw\_frames $X_l = \{x_l^i\}_{i=1}^M$ where the arrival frequency of each raw frame is $F_l$ Hz. Due to the inherent properties of different sensors, $F_l \textgreater F_r$. We further fuses R\_raw\_frames and L\_raw\_frames for vehicle detection task. The fusion and detection frequency is  $F_f$. The ground truth is $Y_i=(y_i, b_i)$, the combination for vehicle label $y_i$ and bounding box coordinates $b_i=(b_i^x, b_i^y, b_i^w, b_i^h)$.


% at the frequency of $F_f$ ($F_r < F_f \leq F_l$) of generating fusion results based on the MVDNet network almost with no loss of precision. The fusion and detection frequency $F_f$ can be dynamically adjusted according to specific needs. The ground truth is $Y_i=(y_i, b_i)$, the combination for vehicle label $y_i$ and bounding box coordinates $b_i=(b_i^x, b_i^y, b_i^w, b_i^h)$ , 

\begin{table*}[]
\centering
\caption{Some basic concepts in this paper}
\label{concept}
\begin{tabular}{ll}
\hline
Item              & Description                                                                       \\ \hline
L\_raw\_frame     & Lidar axis 360 degree point cloud                                                 \\
R\_raw\_frame     & Polar axis 360 degree Radar intensity map                                         \\
ratio             & Numbers of L\_raw\_frame scans during a R\_raw\_frame scan interval             \\ \hline
Index\_L\_frame   & Concatenated previous one and following ratio L\_raw\_frames into one frame        \\
Index\_R\_frame   & Cartesian axis Radar intensity map indexed by the timestamps of the R\_raw\_frame \\ \hline
Paired\_frames    & Paired Index\_L\_frame and Index\_R\_frame                                    \\
H\_Paired\_frames &Including the current and historical (H-1) Paired\_frames                           \\ \hline
\end{tabular}
\end{table*}





\section{RELATED WORK}
%Vehicle Detection using Multiple Sensor
To enhance 3D perception in autonomous driving, many works have proposed to fuse different sensor data modalities to leverage their complementary advantages, including cameras, Lidars and Radars, the three most common sensors used in ADS. 
MVDNet \cite{qian2021robust} proposes fusion model to fuse Lidar and Radar sensors with attention mechanism for vehicle detection in foggy weather and achieves state-of-the-art resutls on the ORR dataset \cite{barnes2020oxford}.
Li et al. \cite{li2022modality} proposes the ST-MVDNet to address the issue of missing sensor data in multi-modal vehicle detection for Lidar and Radar. 
Farag et al. \cite{farag2021real} proposes a real-time road-object detection and tracking method for autonomous driving, which uses a tailored unscented Kalman filter to perform data fusion of Lidar and Radar. LiRaNet \cite{shah2020liranet} is proposed for end-to-end trajectory prediction which utilizes Radar sensor information along with Lidar and high definition maps. 
For camera-Lidar-Radar fusion, Li et al. \cite{li2022mathsf} developes EZFfusion framework for mutli-model 3D object detection and tracking for camera, Lidar and Radar. 
DEF\cite{bijelic2020seeing} proposes an baseline fusion detector with all of the sensors including camera, Lidar, and Radar. 
FUTR3D \cite{chen2022futr3d} is a unified sensor fusion framework, which can be used in almost any sensor configuration. It uses a query-based Modality-Agnostic Feature Sampler, together with a transformer decoder with a set-to-set loss for 3D detection. 
However, existing Lidar/Radar fusion models are developed under the assumption that the Lidar/Radar data are perfectly synchronized in time. If not, downsampling the faster Lidar data at the same frequency as Radar to align them manually \cite{qian2021robust,li2022modality,kim2020low,shah2020liranet,farag2021real,li2022mathsf,bijelic2020seeing,chen2022futr3d}.


For another perspective, some researchers in the real-time area aim to develop the infrastructure-vehicle cooperative autonomous approach to allow sensors to capture environment in real time, and then perform timely fusion and perception \cite{liu2021towards,prakash2021multi,cui2022coopernaut,liu2022brief,he2021vi}.In this paper, we develop techniques to directly fuse temporally unaligned Radar/Lidar data and achieve high output frequency with little accuracy loss.


% %camera-Lidar fusion
% For camera-Lidar fusion, some works constrain the 3D search space with 2D object detection \cite{lahoud20172d,qi2019deep,vora2020pointpainting, kim2018robust, xie2020pi}, while others fuse 2D and 3D features at the task-level \cite{park2021multi, qi2020imvotenet} or feature-level \cite{huang2020epnet, sindagi2019mvx}. MV3D \cite{chen2017multi} processes both Lidar point cloud and RGB images with 2D CNNs for 3D object detection. Liang et al. \cite{liang2019multi} proposes a multi-task multi-sensor detection model that jointly reasons about object detection, ground estimate and depth completion. PointFusion \cite{xu2018pointfusion} combines feature vectors of Lidar and camera to predict 3D boxes of vehicles. Frustum-PointNet \cite{qi2018frustum} and Frustum-ConvNet \cite{wang2019frustum} use 2D object detectors to generate 2D proposals in the camera view, then lift 2D proposals to 3D frustums, and finally use perform 3D box estimation within the frustums.

%{\color{red} Some works about training enhancement.} 






% %camera-Lidar fusion
% For camera-Lidar fusion, some works constrain the 3D search space with 2D object detection \cite{lahoud20172d,qi2019deep,vora2020pointpainting, kim2018robust, xie2020pi}, while others fuse 2D and 3D features at the task-level \cite{park2021multi, qi2020imvotenet} or feature-level \cite{huang2020epnet, sindagi2019mvx}. MV3D \cite{chen2017multi} processes both Lidar point cloud and RGB images with 2D CNNs for 3D object detection. Liang et al. \cite{liang2019multi} proposes a multi-task multi-sensor detection model that jointly reasons about object detection, ground estimate and depth completion. PointFusion \cite{xu2018pointfusion} combines feature vectors of Lidar and camera to predict 3D boxes of vehicles. Frustum-PointNet \cite{qi2018frustum} and Frustum-ConvNet \cite{wang2019frustum} use 2D object detectors to generate 2D proposals in the camera view, then lift 2D proposals to 3D frustums, and finally use perform 3D box estimation within the frustums.

%{\color{red} Some works about training enhancement.} 






table 6
\begin{tabular}{|cc|ccc|ccc|ccc|ccc|ccc|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Model}} & \emph{offset} & \multicolumn{3}{c|}{1}                                                                     & \multicolumn{3}{c|}{2}                                                                     & \multicolumn{3}{c|}{3}                                                                    & \multicolumn{3}{c|}{4}                                                                    & \multicolumn{3}{c|}{5}                                                                     \\ \cline{2-17} 
\multicolumn{1}{|c|}{}                       & IoU         & \multicolumn{1}{c|}{0.5}            & \multicolumn{1}{c|}{0.65}           & 0.8            & \multicolumn{1}{c|}{0.5}            & \multicolumn{1}{c|}{0.65}           & 0.8            & \multicolumn{1}{c|}{0.5}           & \multicolumn{1}{c|}{0.65}           & 0.8            & \multicolumn{1}{c|}{0.5}            & \multicolumn{1}{c|}{0.65}          & 0.8            & \multicolumn{1}{c|}{0.5}            & \multicolumn{1}{c|}{0.65}           & 0.8            \\ \hline
\multicolumn{2}{|c|}{MVDNet\_1}                            & \multicolumn{1}{c|}{\textbf{0.898}} & \multicolumn{1}{c|}{\textbf{0.869}} & \textbf{0.722} & \multicolumn{1}{c|}{0.867}          & \multicolumn{1}{c|}{0.841}          & 0.668          & \multicolumn{1}{c|}{0.847}         & \multicolumn{1}{c|}{0.827}          & 0.652          & \multicolumn{1}{c|}{0.828}          & \multicolumn{1}{c|}{0.809}         & 0.643          & \multicolumn{1}{c|}{0.826}          & \multicolumn{1}{c|}{0.801}          & 0.644          \\ \hline
\multicolumn{2}{|c|}{MVDNet\_2}                            & \multicolumn{1}{c|}{0.87}           & \multicolumn{1}{c|}{0.85}           & 0.67           & \multicolumn{1}{c|}{\textbf{0.899}} & \multicolumn{1}{c|}{\textbf{0.877}} & \textbf{0.724} & \multicolumn{1}{c|}{0.889}         & \multicolumn{1}{c|}{0.863}          & 0.684          & \multicolumn{1}{c|}{0.876}          & \multicolumn{1}{c|}{0.848}         & 0.705          & \multicolumn{1}{c|}{0.868}          & \multicolumn{1}{c|}{0.847}          & 0.702          \\ \hline
\multicolumn{2}{|c|}{MVDNet\_3}                            & \multicolumn{1}{c|}{0.867}          & \multicolumn{1}{c|}{0.846}          & 0.699          & \multicolumn{1}{c|}{0.868}          & \multicolumn{1}{c|}{0.847}          & 0.701          & \multicolumn{1}{c|}{\textbf{0.89}} & \multicolumn{1}{c|}{\textbf{0.867}} & \textbf{0.722} & \multicolumn{1}{c|}{0.879}          & \multicolumn{1}{c|}{0.858}         & 0.709          & \multicolumn{1}{c|}{0.878}          & \multicolumn{1}{c|}{0.849}          & 0.7            \\ \hline
\multicolumn{2}{|c|}{MVDNet\_4}                            & \multicolumn{1}{c|}{0.877}          & \multicolumn{1}{c|}{0.855}          & 0.686          & \multicolumn{1}{c|}{0.881}          & \multicolumn{1}{c|}{0.853}          & 0.683          & \multicolumn{1}{c|}{0.874}         & \multicolumn{1}{c|}{0.853}          & 0.688          & \multicolumn{1}{c|}{\textbf{0.888}} & \multicolumn{1}{c|}{\textbf{0.86}} & \textbf{0.709} & \multicolumn{1}{c|}{0.875}          & \multicolumn{1}{c|}{0.854}          & 0.688          \\ \hline
\multicolumn{2}{|c|}{MVDNet\_5}                            & \multicolumn{1}{c|}{0.855}          & \multicolumn{1}{c|}{0.833}          & 0.679          & \multicolumn{1}{c|}{0.862}          & \multicolumn{1}{c|}{0.834}          & 0.687          & \multicolumn{1}{c|}{0.865}         & \multicolumn{1}{c|}{0.843}          & 0.689          & \multicolumn{1}{c|}{0.884}          & \multicolumn{1}{c|}{0.864}         & 0.704          & \multicolumn{1}{c|}{\textbf{0.885}} & \multicolumn{1}{c|}{\textbf{0.865}} & \textbf{0.707} \\ \hline
\end{tabular}
